Competing Bandits in Matching Markets

Stable matching, a classical model for two-sided markets, has long been studied with little consideration for how each side's preferences are learned. With the advent of massive online markets powered by data-driven matching platforms, it has become necessary to better understand the interplay between learning and market objectives. We propose a statistical learning model in which one side of the market does not have a priori knowledge about its preferences for the other side and is required to learn these from stochastic rewards. Our model extends the standard multi-armed bandits framework to multiple players, with the added feature that arms have preferences over players. We study both centralized and decentralized approaches to this problem and show surprising exploration-exploitation trade-offs compared to the single player multi-armed bandits setting.

==> centralized_setting.tex <==
% !TeX root = main.tex 
\newpage
 
\section{Problem Settings}


We conside a multi armed bandit problem with $N$ agents and $K$ stochastic arms. More precisely, when a agent $i$ successfully pulls arm $j$ she receives a stochastic reward $X_{t, J_t}^{(i)}$ which is sampled from a $\sigma$-sub Guassian distribution with mean $\mu^{(i)}_{J_t}$ ($J_t \in \RR^{K}$ is a random vector containing the arms chosen by  all the agents at time $t$, i.e. $J_{t, i}$ denotes the arm chosen by agent $i$ at time t). For each fixed agent $i$ we assume $\mu^{(i)}_{j} \neq \mu^{(i)}_{j^\prime}$ for all $j \neq j^\prime $ in $[K]$.

We study a competitive setting for the agents in which each arm has preferences over agents. Namely, arm $j$ has a ranking $\pi_j(i)$ for each agent $i$, where $\pi_j$ is a permutation of $[N]$. Then, if two agents $i$ and $i^\prime$ select the same arm, the arm awards the stochastic reward to the agent ranked higher, i.e. to $i$ if $\pi_j(i) > \pi_j(i^\prime)$ or to $i^\prime$ if $\pi_j(i) < \pi_j(i^{\prime})$. Each agent knows all the arm rankings $\pi_i$ of the other agents. This assumption is not limiting; because the conflicts are resolved deterministically, the agents can determine all the rankings $\pi_i$ in constant time. 

We are now ready to define a notion of regret natural to this problem. If all the agents knew each others expected rewards $\mu^{(i)}_{j}$, they would each sample the agent optimal stable matching, where the arms are ordered by the reward they provide. Let $\mu^{(i)}_\star$ denote the agent optimal stable match of agent $i$. Then, we define the pseudo-regret of agent $i$ to be
\begin{align*}
R^{(i)}(T) = T \mu^{(i)}_\star - \sum_{t = 1}^T \EE X^{(i)}_{t, J_t}. 
\end{align*}

In order to fully specify the problem we need to clarify what information the agents have access to. We consider three settings.
 

\paragraph{Full Information (Centralized).} We assume that after each time steps agents can see the actions of all the other agents, the results of the ensuing conflicts, and the rewards each agent acquires. Then, agents could infer the current preferences other agents have for different arms and plan accordingly when choosing the next arm. 

Alternatively, we can think of each agent submitting their current preferences over arms to a central authority. Then, the central authority runs the Gale-Shapley algorithm with the preferences it received and sends back to each agent their optimal stable match corresponding to all the current preferences.

\paragraph{Partial Information.} Agents can see each others actions and the ensuing conflicts. However, agents cannot cannot see the rewards other agents receive.

\paragraph{No Information.} After selecting an arm, agents can tell whether they lost a conflict on that arm. If they successfully sampled an arm, they observe their own reward. However, they do not observe any other information. In particular, they do not know what actions other agents are playing.

\subsection{Full information / Centralized}

Algorithm~\ref{alg:central_ucb} is natural. Our aim is twofold: we wish to show that this algorithm achieves $\Ocal(\log(T))$ regret for each agent, and wish to study whether one agent has an incentive to follow this algorithm when all other agents are following it. More precisely,
an agent could submit arbitrary rankings $\gamma_{i,t}$ to the central authority and could play arbitrary actions, disregarding the proposal of the central authority. Do agents have an incentive to take advantage of this liberty? 

\begin{algorithm}
\caption{Centralized GS-UCB}\label{alg:central_ucb}
\begin{algorithmic}[1]
	\FOR{$t = 0, 1, \ldots, T $}
        \STATE Each agent $i$ ranks the arms according to the upper confidence bounds $U^{(i)}_{t, j}$ and ties are broken uniformly at random. Then, if $U^{(i)}_{t, j} > U^{(i)}_{t, j^\prime}$, agent $i$ assigns ranks $\gamma^{(i)}_{t}(j) > \gamma^{(i)}_{t}(j^\prime)$.
        \STATE Agent $i$ sends the ranking $\gamma^{(i)}_{t}$ to the central authority.
        \STATE The central authority runs the GS algorithm with the preferences $\gamma^{(1)}_{t}$, $\gamma^{(2)}_{t}$, \ldots, $\gamma^{(N)}_{t}$, $\pi_{1}$, $\pi_{2}$, \ldots, $\pi_{K}$.
        \STATE The central authority sends proposed actions $P_t$ to the agents, where $P_t$ is a vector with the $i$-th entry containing the stable match of agent $i$ at time $t$. 
        \STATE The agents play the actions $P_t$. Each agent $i$ receives reward $X^{(i)}_{t, P_t}$.
        \STATE Each agent updates the upper confidence bound for arm $P_{t, i}$ according to the reawrd $X^{(i)}_{t, P_t}$ (if an arm has not been pulled yet, its upper confidence bound is infinity).
        \ENDFOR
\end{algorithmic}
\end{algorithm}

==> experiments.tex <==
% !TeX root = main.tex 
\section{Experiments}

\subsection{Global preferences}

In Figures \ref{fig:ucb_global} and \ref{fig:ucbca_global}, we can see the results from running the usual UCB algorithm and the conflict avoiding UCB on a market with global preferences. Stability is not achieved by the usual UCB algorithm---less than half of the matches are stable after 100,000 rounds.

On the other hand, the conflict avoiding UCB achieves stability. All agents attain low stable regret after less than 10,000 rounds.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=\textwidth, trim=100 100 100 100, clip]{globalmkt_ucb_numagents20_variance1-00.png}
	\caption{Running usual UCB on a market of 20 agents, 20 arms. Each side has global preferences over the other. }\label{fig:ucb_global}
\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=\textwidth, trim=100 100 100 100, clip]{globalmkt_ucb_conf_avoid_numagents20_variance1-00.png}
	\caption{Running conflict avoiding UCB on a market of 20 agents, 20 arms. Each side has global preferences over the other. }\label{fig:ucbca_global}
\end{figure}

\subsection{Idiosyncratic preferences}

Figure \ref{fig:ucbca_idio} shows the results from running UCB conflict avoiding on a market with idiosyncratic two sided preferences.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=\textwidth, trim=100 100 100 100, clip]{idiomkt_ucb_numagents20_variance1-00.png}
	\caption{Running usual UCB on a market of 20 agents, 20 arms. Each side has idiosyncratic preferences over the other. }\label{fig:ucb_idio}
\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=\textwidth, trim=100 100 100 100, clip]{idiomkt_ucb_conf_avoid_numagents20_variance1-00.png}
	\caption{Running conflict avoiding UCB on a market of 20 agents, 20 arms. Each side has idiosyncratic preferences over the other. }\label{fig:ucbca_idio}
\end{figure}


==> explore_then_propose.tex <==
% !TeX root = main.tex 
\section{Explore then Propose algorithm}

This is a baseline algorithm that achieves stability with idiosyncratic preferences.

In stage 1, all agents explore all arms uniformly at random. Agents update their sample means of arms if the pull was successful.

In stage 2, each round each agent proposes to the arm with the highest sample mean that they haven't been rejected by (in this stage).

Proof:

Suppose stage $1$ lasts $T$ rounds.
Fix the agent. 
For any particular attempt on an arm, let $Y$ denote the event of a successful pull. The probability of a successful pull is bounded from below by the probability of a successful pull for an agent that is the least preferred by the arm attempted.
\[ \Pr\{Y = 1\} \geq \left( \frac{M-1}{M} \right)^N \]

Let $Y_i$ be the event that arm $i$ is pulled successfully in any round.
\[ \Pr\{ Y_i=1 \} \geq \frac{1}{M} \left( \frac{M-1}{M} \right)^N =: p(M,N) \]

Let $T_i$ be the number of times arm $i$ was pulled. $T_i \sim Binom(T, p(M,N))$. We can use a standard tail bound:
\[ \Pr\{ T_i \leq t \} \leq \exp(-2\frac{(Tp-t)^2}{T}) \]

Stage 2 gives rise to a matching that is stable according to the order of the learned preferences ($\hat{R}^i_j$), after $N$ rounds. This is because, at least one agent is matched successfully at every round.

If any agent $j$ (matched to arm $k$) is part of a blocking pair with arm $i$ (according to true preferences, $r^i_j$ ), we must have $\hat{R}^k_j > \hat{R}^i_j $ and $r^i_j > r^k_j $. Therefore, we need to bound the tail probability:
\[ \Pr\{(\hat{R}^i_j -\hat{R}^k_j  ) - (r^i_j -r^k_j) \leq -( r^i_j - r^k_j)   \} \leq e^{} \]

Then union bound over all possible blocking pairs.

==> problem_setting.tex <==
% !TeX root = main.tex 
\section{Problem Setting}

\begin{itemize}
\item $N$ agents: each agent $j$ gets (random) reward $R_j^i > 0$ from arm $i$, if accepted by the arm pulled. If rejected by arm pulled, agent gets $0$ reward. $\E[R_j^i] = r_j^i$. 
\item $M$ arms: each arm $i$ knows its preference $p_i^j > 0$ for agent $j$. If pulled by more than one agent in one round, the arm only accepts one agent $j$ with the highest $p_i^j$.
\end{itemize}

~


\textbf{Question:} What algorithm (used by the agents) leads to a stable matching with high probability?

Key difference from Stable Matching/Auctions/Mechanism Design literature is that agents don't initially know their utilities from each arm and have to learn it via interaction.

We introduce a new notion of player regret that is the difference between the agent's average reward, $\frac{1}{n} \sum_{t=1}^n-R^{i_t}_t$, and the reward that the agent would have received from the arm that they are matched to in the unique agent-optimal stable matching, $R^k$:
\[ \tilde{\calR}\su{k}_n =R^k - \frac{1}{n} \sum_{t=1}^n-R^{i_t}_t \]

==> ucb_conflict_avoiding.tex <==
% !TeX root = main.tex 
\section{UCB conflict avoiding algorithm}

\begin{algorithm}
\caption{UCB conflict avoiding}\label{alg:ucb_conflict_avoid}
\begin{algorithmic}[1]
	\renewcommand{\algorithmicrequire}{\textbf{Input: }}
	\renewcommand{\algorithmicensure}{\textbf{Output: }}
	\REQUIRE 
	\FOR{$t = 0, 1, \ldots, T $}
		\FOR{$j = 1, \ldots, N $}
			\STATE Update plausible set $P_j$ for agent $j$: an arm $a$ is plausible if of all the agents who has won a conflict on $a$ against $j$, none of them chose $a$ at time $t-1$.
			\STATE Pulls $a \in P_j$ with maximum upper confidence bound
			\IF{$j$ wins conflict}
			\STATE Update upper confidence bound for arm $a$.
			\ENDIF
		\ENDFOR
	\ENDFOR
	\STATE \textbf{return} $\x_T$
\end{algorithmic}
\end{algorithm}
\lnote{check if the written algorithm is the same as what we implemented? if not, change the written version.}

An issue with this algorithm is that it will not lead to the agent-optimal matching, considering a simple 2 x 2 example, where any matching is a stable matching. The conflict set mechanism causes agents to only exploit the arms that are sub-optimal for them, even though this is a stable matching.

\begin{lemma}[Bound on number of non-stable pulls, global preferences]
	Let $N\su{j}(n)$ denote the number of times after $n$ rounds that agent $j$ pulled an arm that is not its stable arm (i.e. arm with the $j$-th ranking). 	Let $T_i\su{k}(n)$ is the number of times arm $i$ was pulled successfully by agent $k$ and $T\su{k}_\emptyset(n)$ the number of times agent $k$ lost a conflict, after $n$ rounds. Note that by definition, \[\sum_{j\neq i} T_i\su{j}(n) = N\su{j}(n).\]
	Then, we have
	\begin{equation}\label{eq:non-stable-pulls}
	N\su{k}(n) \leq \sum_{i = k+1}^M T\su{k}_i(n) + \sum_{j=1}^{k-1}(N\su{i}(n) + T_\emptyset\su{i}(n) )~ \text{, and~}
	\end{equation}
	
	\begin{equation}\label{eq:non-stable-pulls2}
	N\su{k}(n) \leq \sum_{j \leq k}\sum_{i > j} T\su{j}_i(n)  +\sum_{j \leq k}(k-j) T\su{j}_\emptyset(n) 
	\end{equation}
	\begin{equation}\label{eq:non-stable-pulls3}
	\sum_{j\leq k} N\su{j}(n) \leq \sum_{j \leq k}\sum_{i > j} T\su{j}_i(n)  +\sum_{j \leq k-1} \left(T\su{j}_\emptyset(n) + N\su{j}(n)\right)
	\end{equation}
	
	\begin{equation}\label{eq:non-stable-pulls4}
	\sum_{j\leq k} N\su{j}(n) \leq \sum_{j\leq k} (k-j+1) \sum_{i > j} T_i\su{j}(n) +  \sum_{i \leq k-1} (k-i) T_\emptyset\su{i}(n)
	\end{equation}
\end{lemma}
\begin{proof}
%	We proceed by induction. First, for the base case, we consider the first-ranked agent. Since $T_\emptyset\su{1} = 0$ (agent 1 always wins a conflict), \eqref{eq:non-stable-pulls} is satisfied with equality, that is,
%	\[N\su{1}(n) = \sum_{i = 2}^M T\su{1}_i(n)  \]
%	Now we assume \eqref{eq:non-stable-pulls} holds for agent $k$ and argue that correctness of the inductive step. 
First we argue that correctness of \eqref{eq:non-stable-pulls}. If agent $k$ did not pull its stable arm, it must have (i) lost a conflict on the arm it attempted, (ii) pulled a better ranked arm and won the conflict (therefore a better ranked agent must have not pulled its stable arm that round), or (iii) pulled a worse ranked arm and won the conflict. For case (ii), we use the inequality, $T_i\su{k}(n) \leq \sum_{j\neq i} T_i\su{j}(n) \leq N\su{i}(n) + T_\emptyset\su{i}(n) $.

 Therefore, we have:
	\begin{align*}
	N\su{k}(n) &\leq \sum_{i = k+1}^M T\su{k}_i(n) + \sum_{i = 1}^{k-1} T\su{k}_i(n) \\
	&\leq \sum_{i = k+1}^M T\su{k}_i(n) + \sum_{i=1}^{k-1}(N\su{i}(n) + T_\emptyset\su{i}(n) ) \tag{proving \eqref{eq:non-stable-pulls2}}\\
	&= \sum_{i > k} T\su{k}_i(n) +\sum_{i < k}T_\emptyset\su{i}(n) + N\su{k-1}(n)+\sum_{i < k-1}N\su{i}(n) \\
	&\leq \sum_{i > k} T\su{k}_i(n) +\sum_{i < k}T_\emptyset\su{i}(n) + \sum_{i > k-1} T\su{k-1}_i(n) + \sum_{i < k-1}(N\su{i}(n) + T_\emptyset\su{i}(n) ) +\sum_{i < k-1}N\su{i}(n)\tag{applying \eqref{eq:non-stable-pulls}} \\
	&= \sum_{i > k} T\su{k}_i(n) +\sum_{i < k}T_\emptyset\su{i}(n) + \sum_{i > k-1} T\su{k-1}_i(n) + \sum_{i < k-1} T_\emptyset\su{i}(n)+ 2\sum_{i < k-1}N\su{i}(n) \\
	&\leq \sum_{j \leq k}\sum_{i > j} T\su{j}_i(n)  + \sum_{j \leq k}\sum_{i < j} T\su{i}_\emptyset(n)  \tag{applying previous 2 steps repeatedly} \\
	&\leq \sum_{j \leq k}\sum_{i > j} T\su{j}_i(n)  +\sum_{j \leq k}(k-j) T\su{j}_\emptyset(n) \tag{proving \eqref{eq:non-stable-pulls2}}
	\end{align*}
	
	To prove \eqref{eq:non-stable-pulls3}:
	\begin{align*}
	\sum_{j\leq k} N\su{j}(n) &\leq \sum_{j\leq k} \sum_{i > j} T_i\su{j}(n) + \sum_{j\leq k} \sum_{i < j} T_i\su{j}(n) \\
	&\leq \sum_{j\leq k} \sum_{i > j} T_i\su{j}(n) + \sum_{i < k}\sum_{j > i} T_i\su{j}(n) \\
	&\leq \sum_{j\leq k} \sum_{i > j} T_i\su{j}(n) + \sum_{i < k}\sum_{j \neq i} T_i\su{j}(n) \\
	&\leq \sum_{j\leq k} \sum_{i > j} T_i\su{j}(n) + \sum_{i \leq k-1} N\su{i}(n) + T_\emptyset\su{i}(n) \tag{proving \eqref{eq:non-stable-pulls3}}\\
	&\leq \sum_{j\leq k} \sum_{i > j} T_i\su{j}(n) +  \sum_{i \leq k-1}  T_\emptyset\su{i}(n) + \sum_{j\leq k-1} \sum_{i > j} T_i\su{j}(n) + \sum_{i \leq k-2} N\su{i}(n) + T_\emptyset\su{i}(n) \tag{applying \eqref{eq:non-stable-pulls3}}\\
	&\leq \sum_{j\leq k} (k-j+1) \sum_{i > j} T_i\su{j}(n) +  \sum_{i \leq k-1} (k-i) T_\emptyset\su{i}(n) \tag{applying \eqref{eq:non-stable-pulls3} repeatedly} 
	\end{align*}
\end{proof}

\begin{lemma}
	We would like to give a closed form expression for $T_\emptyset\su{k}(n)$ in terms of $T_i\su{j}$ where $j \leq k$ and $i > j$. 
	\end{lemma}
	\begin{proof}
		We use the following two inequalities. The first one is \eqref{eq:non-stable-pulls4}:
		\[	\sum_{j\leq k} N\su{j}(n) \leq \sum_{j\leq k} (k-j+1) \sum_{i > j} T_i\su{j}(n) +  \sum_{i \leq k-1} (k-i) T_\emptyset\su{i}(n), \]
		which relates the number of non-stable pulls by agent $k$ to the number of suboptimal pulls (pulling an arm that is worse than their stable arm) by agents that are at least as highly ranked as $k$ and the number of conflicts lost by agents that are better than $k$.
		The second one is \[ T_\emptyset\su{k}(n) \leq \sum_{j<k} (2N\su{j}(n) + T_\emptyset\su{j}(n)) + (k-1)M, \]
		which relates the number of conflicts lost by agent $k$ to the number of non-stable pulls by better agents and the number of conflicts lost by better agents. 
		We have for the base case:
		\[ N\su{1}(n) = \sum_{i=2}^M T_i\su{1}(n); ~T_\emptyset\su{1} = 0 \]
		
		We have the recurrence:
		\begin{equation}
		T_\emptyset\su{k+1}(n) \leq 2\sum_{j\leq k} (k-j+1) \sum_{i > j} T_i\su{j}(n) +  2\sum_{i \leq k-1} (k-i) T_\emptyset\su{i}(n) + \sum_{j\leq k} T_\emptyset\su{j}(n) + kM
		\end{equation}
		Unfortunately this bound definitely incurs an exponential dependence in the rank of the agent, $k$; this is already true for any recurrence of the form $f_{k+1} \leq 2 f_{k}$.
	\end{proof}

\begin{theorem}[Agents have global preferences over arms and arms have global preferences over agents]\label{thm:ucbca_global}
Assume $R^i_j = R^i$ (all agents get the same reward from arm $i$) and $p_i^j = p^j$ (all agents have the same preference for agent $j$). In this case, the stable matching is unique. Then Algorithm \ref{alg:ucb_conflict_avoid} achieves ...
\end{theorem}
\begin{proof}
	The highest ranked agent wins all conflicts so gets the usual UCB regret (which is?).
	The $k$-th ranked agent's performance depends on all better ranked agents acting optimally with high probability.
	
	Let $i_t$ be (random) index of the arm pulled by $k$-th ranked agent time $t$. Let $R^{i}_t$ be the reward of arm $i$ at time $t$ for agent $k$. If the pull was unsuccessful, $i_t = \emptyset$ and define the reward $R_{\emptyset} = 0$.
	
	For the $k$-th ranked agent, total regret with respect to its stable match after $n$ rounds is
	\begin{align*}
	\tilde{\calR}\su{k}_n &= \sum_{t=1}^n(R_t^k-R^{i_t}_t ),
	\end{align*}
	Let $T_i\su{k}(n)$ is the number of times arm $i$ was pulled successfully by agent $k$ and $T\su{k}_\emptyset(n)$ the number of times agent $k$ lost a conflict, after $n$ rounds. Let $\Delta\su{k}_i$ denote $r^i_k - r^k_k$ for arm $i$, and $\Delta\su{k}_\emptyset$ denote $-r^k_k$.
	The expected total regret can be written as:
	\begin{align*}
	\calR_n^{(k)} &= \Delta\su{k}_\emptyset \E[T^{(k)}_\emptyset(n)]+ \sum_{i\neq k} \Delta\su{k}_i\E[T\su{k}_i(n)]
	\end{align*}
	
	We only need to bound $\E[T_\emptyset(n)]$ and $\E[T_i(n)]$ for $i: \Delta_i\su{k} > 0$.
	
Let $A^{(k)}_t$ denote the arm attempted by agent $k$ at time $t$. We analyze the problem for $k = 2$ first. Let $C\su{2}_{1, i}(n) = \sum_{t=1}^n  \Ind{A_t\su{1}=A_t\su{2}=i}$ be the number of times agent 1 and agent 2 conflicted on arm $i$ by time $n$.
	
	\begin{align*}
	T\su{2}_\emptyset(n) &= \sum_{t=1}^n \Ind{A\su{2}_t = \emptyset} \\
	&=\sum_{t=1}^n \sum_{i=1}^M \Ind{A_t^{(1)}=i}\Ind{A_t^{(2)}=i} \tag{conflict must be with 1st-ranked agent}\\
	&=\sum_{t=1}^n \sum_{i=1}^M \Ind{A_t^{(1)}=i}\Ind{A_t^{(2)}=i}\left(\Ind{A_{t-1}^{(1)}\neq i}\Ind{	C\su{2}_{1, i}(t) > 0} +\Ind{	C\su{2}_{1, i}(t) = 0} \right) \tag{potential set}\\
	&\leq \sum_{t=1}^n \sum_{i=1}^M \Ind{A_t^{(1)}=i}\Ind{A_t^{(2)}=i}\Ind{A_{t-1}^{(1)}\neq i}+\sum_{i=1}^M \sum_{t=1}^n  \Ind{A_t\su{1}=A_t\su{2}=i} \Ind{	C\su{2}_{1, i}(t) = 0}  \\
	&\leq \sum_{t=1}^n \sum_{i=1}^M \Ind{A_t^{(1)}=i}\Ind{A_t^{(2)}=i}\Ind{A_{t-1}^{(1)}\neq i} + M\\
	&\leq \sum_{t=1}^n \Ind{A_t^{(1)}\neq A_{t-1}^{(1)} } + M \tag{Agent 1 switched arms}\\
	&\leq \sum_{t=1}^n \Ind{A_{t}^{(1)}\neq 1} +  \Ind{A_{t-1}^{(1)}\neq 1} + M \tag{Agent 1 didn't pull best arm} \\
	&\leq 2\sum_{i=2}^M T_i\su{1}(n) + M
		\end{align*}
		Hence we have the inequality \[ \E[T\su{2}_\emptyset(n)]  \leq C \sum_{i=2}^M \E[T_i\su{1}(n)] \leq C\sum_{i=2}^M \frac{\log(n)}{{\Delta_i^{(1)}}^2} \]
		where the last inequality is from a standard analysis of the UCB algorithm.
		
		Now we turn to bounding $T_i\su{2}(n)$ for $i > 2$. Note that $ A_t\su{k}= i \implies $ $i$ is in the potential set for agent $k$ at time $t$. Since agent $k$ can lose conflicts with at most $k-1$ agents (because it is globally the $k$-th ranked agent), the potential set for agent $k$ must have size at least $M-k+1$, so it must contain an arm whose mean reward is at least as high as arm $k$. This implies $i$ must not be the best arm in the potential set, so it must have UCB larger than the best arm in the potential set (which we denote $*_t$). 
		
		Let $\hat{\mu}\su{k}_i(t-1)$ denote the sample average of arm $i$ for agent $k$ at time $t-1$.
		\begin{align*}
		T_i\su{k}(n) &\leq \sum_{t-1}^n \Ind{A_t\su{k}= i} \\
		&\leq \sum_{t-1}^n \Ind{\hat{\mu}\su{k}_{*_t}(t-1) + \sqrt{\frac{2\log f(t)}{T\su{k}_{*_t}(t-1)} }\leq R\su{k}_{*_t }-\epsilon } \\&\quad + \Ind{\hat{\mu}\su{k}_i(t-1) + \sqrt{\frac{2\log f(t)}{T\su{k}_i(t-1)} } \geq R\su{k}_{*_t }-\epsilon \text{ and }A_t\su{k}= i} 
		\end{align*}
		By a standard analysis of UCB (which takes a union bound over all possible values of $T\su{k}_{*_t}(t-1)$), with the right choice of $f$, we have :
		\begin{align*}
	\E\left[\sum_{t-1}^n \Ind{\hat{\mu}\su{k}_{*_t}(t-1) + \sqrt{\frac{2\log f(t)}{T\su{k}_{*_t}(t-1)} }\leq R\su{k}_{*_t }-\epsilon } \right] &\leq 5/\epsilon^2
		\end{align*}
		For the other term, we have 
		\begin{align*}
		&\E\left[\Ind{\hat{\mu}\su{k}_i(t-1) + \sqrt{\frac{2\log f(t)}{T\su{k}_i(t-1)} } \geq R\su{k}_{*_t }-\epsilon \text{ and }A_t\su{k}= i} \right] \\
		\leq &\E\left[\Ind{\hat{\mu}\su{k}_i(t-1) + \sqrt{\frac{2\log f(t)}{T\su{k}_i(t-1)} } \geq R\su{k}_k-\epsilon \text{ and }A_t\su{k}= i} \right] \tag{best arm in potential set at least as good as arm $k$} \\
		\leq & 1+ \frac{2}{ (\Delta\su{k}_i - \epsilon)^2}(\log f(n) +\sqrt{\pi \log f(n)}+1)
		\end{align*}
		
		Hence, by standard arguments for UCB again, we have for all $i < k$, 
		\begin{equation}\label{eq:subopt}
		\E[T_i\su{k}(n) ] \leq C\frac{\log(n)}{(\Delta\su{k}_i )^2} 
		\end{equation} 
		
		To summarize, for the 2nd ranked agent, we have the following bound on average regret:
		\begin{equation}
		\calR_n\su{2} \leq C \Delta\su{k}_\emptyset \sum_{i=2}^M \frac{\log(n)}{{\Delta_i^{(1)}}^2} + C\sum_{i: \Delta_i\su{k} > 0} \frac{\log(n)}{\Delta\su{k}_i }
		\end{equation}
		
		\lnote{Above: Could get a bound that doesn't depend on suboptimality gaps.}
		
		Now, we need to consider $k>2$. First we need to bound $T\su{k}_\emptyset(n) $ in terms of the actions of all better ranked agents. 
		
		\begin{align*}
		T\su{k}_\emptyset(n) &= \sum_{t=1}^n \Ind{A\su{k}_t = \emptyset} \\
		&=\sum_{t=1}^n \sum_{i=1}^M\sum_{j=1}^{k-1} \Ind{A_t^{(j)}=i}\Ind{A_t^{(k)}=i} \tag{conflict must be with better-ranked agent}\\
		&=\sum_{t=1}^n \sum_{i=1}^M\sum_{j=1}^{k-1} \Ind{A_t^{(j)}=i}\Ind{A_t^{(k)}=i} \left(\Ind{A_{t-1}^{(j)}\neq i}\Ind{C\su{k}_{j, i}(t) >0  } + \Ind{C\su{k}_{j, i}(t) =0  }\right)\tag{potential set}\\
			&\leq \sum_{t=1}^n \sum_{i=1}^M\sum_{j=1}^{k-1} \Ind{A_t^{(j)}=i}\Ind{A_t^{(k)}=i} \Ind{A_{t-1}^{(j)}\neq i} + \sum_{i=1}^M\sum_{j=1}^{k-1}\sum_{t=1}^n \Ind{A_t^{(j)}=A_t^{(k)}=i}\Ind{C\su{k}_{j, i}(t) =0  }\\
		&\leq \sum_{t=1}^n \sum_{j=1}^{k-1} \Ind{A_t\su{j}\neq A_{t-1}\su{j}} + (k-1)M \tag{Agent j switched arms}\\
		&\leq \sum_{t=1}^n\sum_{j=1}^{k-1}  \Ind{A_{t}\su{j}\neq j, A_{t}\su{j}\neq \emptyset} +  \Ind{A_{t-1}\su{j}\neq j}+ (k-1)M  \tag{Agent j didn't pull arm j} \\
		&\leq \sum_{j=1}^{k-1} (2N\su{j}(n) + T_\emptyset\su{j}(n))+ (k-1)M 
		\end{align*}
		
		\lnote{We only have a bound on $T_i\su{j}(n)$ for $i > j$ \eqref{eq:subopt}, but not for $i < j$.}
\end{proof}



Next step: extend Theorem \ref{thm:ucbca_global} to
\begin{itemize}
	\item Agents have idiosyncratic preferences over arms (easy?)
	\item Arms also have idiosyncratic preferences over agents (hard)
\end{itemize}

\subsection{Why UCB doesn't work}

\begin{example}
	Consider two agents and three arms. The reward on the worst arm is large enough that once an agent gets a conflict (zero reward) on a better arm, it takes exponentially long for the UCB of the better arm to beat the UCB of the worst arm.
	
	arms = (8, 4, 2), rewards with variance 1
	UCB for arm 3 for agent 2 is $\approx 0 + \sigma \sqrt{2}$ which is smaller than mean for arm 3.
\end{example}
